Efficient simulation of inclusions and reinforcement bars with the isogeometric Boundary Element method

The paper is concerned with the development of efficient and accurate solution procedures for the isogeometric boundary element method (BEM) when applied to problems that contain inclusions that have elastic properties different to the computed domain. This topic has been addressed in previous papers but the approach presented here is a considerable improvement in terms of efficiency and accuracy. One innovation is that initial stresses instead of body forces are used. This then allows a one step solution without iteration. In addition, a novel approach is used for the computation of strains, that avoids the use of highly singular fundamental solutions. Finally, a new type of inclusion is presented that can be used to model reinforcement bars or rock bolts and where analytical integration can be used. Test examples, where results are compared with Finite Element simulations, show that the proposed approach is sound.

==> iabem-macros.tex <==
\usepackage[utf8]{inputenc}
\usepackage[a4paper,twoside,bindingoffset=1cm,head=15pt,body={17cm,25cm},top=2.5cm]{geometry}
\usepackage{amsmath,amssymb}
\usepackage{graphicx}
\usepackage{color}
\usepackage{cite}
\usepackage{ifthen}
\usepackage{titlesec}
\usepackage{fancyhdr}

\setlength{\columnsep}{3em}
\titleformat{\section}{\normalfont\bfseries}{\thesection}{1em}{}
\titlespacing*{\section}{0pt}{*1.5}{1ex}



\newcommand{\todo}[1]{\textcolor{red}{\#\#\# #1 \#\#\#}}

\newcounter{authorcounter}

\newcommand{\iabemauthorlist}{}
\newcommand{\iabemaddresslist}{}
\newcommand{\iabememail}{}
\newcommand{\iabemfootnotes}{}
\newcommand{\iabemauthorpre}{}

\def\theNumberTest#1{%
  \if\relax\detokenize\expandafter{\romannumeral-0#1}\relax
    true%
  \else
    false%
  \fi
}

\newcommand{\iabemspeaker}[3][noemail]{%
    \ifthenelse{\value{authorcounter} > 1}{%
      \renewcommand{\iabemauthorpre}{, }%
    }{%
      \renewcommand{\iabemauthorpre}{}%
    }%
    \ifthenelse{\equal{#1}{noemail}}{%
      \renewcommand{\iabemfootnotes}{}
    }{%    
      \renewcommand{\iabememail}{$^\ast$Email: #1}%
      \renewcommand{\iabemfootnotes}{, \ast}
    }%
    \ifthenelse{\equal{\theNumberTest{#3}}{true}}{%
      \edef\iabemauthorlist{\iabemauthorlist%
        \iabemauthorpre{}\underline{#2}$^{#3\iabemfootnotes%
        }$%
      }%
    }{%    
      \edef\iabemauthorlist{\iabemauthorlist%
        \iabemauthorpre\underline{#2}$^{\arabic{authorcounter}\iabemfootnotes%
        }$%
      }
      \edef\iabemaddresslist{\iabemaddresslist% 
        \par%
        $^{\arabic{authorcounter}}$#3%
      }%      
      \stepcounter{authorcounter}%
    }%
  \ignorespaces
}

\newcommand{\iabemauthor}[3][noemail]{%
    \ifthenelse{\value{authorcounter} > 1}{%
      \renewcommand{\iabemauthorpre}{, }%
    }{%
      \renewcommand{\iabemauthorpre}{}%
    }%
    \ifthenelse{\equal{#1}{noemail}}{%
      \renewcommand{\iabemfootnotes}{}
    }{%    
      \renewcommand{\iabememail}{$^\ast$Email: #1}%
      \renewcommand{\iabemfootnotes}{, \ast}
    }%
    \ifthenelse{\equal{\theNumberTest{#3}}{true}}{%
      \edef\iabemauthorlist{\iabemauthorlist%
        \iabemauthorpre{}#2$^{#3\iabemfootnotes%
        }$%
      }%
    }{% 
      \edef\iabemauthorlist{\iabemauthorlist%
         \iabemauthorpre{}#2$^{\arabic{authorcounter}\iabemfootnotes%
         }$%
      }
      \edef\iabemaddresslist{\iabemaddresslist%
        \par%
        $^{\arabic{authorcounter}}$#3%
      }%
      \stepcounter{authorcounter}%
    }%
  \ignorespaces
}

\newenvironment{iabempaper}[3]{%
  \renewcommand{\iabemauthorlist}{}%
  \renewcommand{\iabememail}{}%
  \setcounter{authorcounter}{1}%
     #2
%  \twocolumn[
    \begin{center}
     \bfseries
     #1
     \bigskip

     \iabemauthorlist
     \mdseries
     \smallskip

     \iabemaddresslist
     \smallskip
 
     \iabememail
 
     \end{center}%
 % ]

}{%
}


% set up headers and footers
\pagestyle{fancy}
% \renewcommand{\chaptermark}[1]{\markboth{#1}{}}
% \renewcommand{\sectionmark}[1]{\markright{\thesection\ #1}}
\fancyhf{}
\fancyhead[LE,RO]{\bfseries}
\fancyhead[LO]{\bfseries FWF Proposal sketch}
\fancyhead[RE]{\bfseries FWF Proposal sketch}
\renewcommand{\headrulewidth}{0.5pt}
\renewcommand{\footrulewidth}{0.5pt}
\fancypagestyle{plain}{%
  \fancyhead{}
%  \renewcommand{\headrulewidth}{0pt}
}


==> settings/myheadings.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % myheadings.tex
% %
% % 	requires:		\usepackage{scrpage2}
% % 				\usepackage{setspace}
% %

%%% Headings
%\pagestyle{headings}
\automark[chapter]{section}
\pagestyle{scrheadings}
% \rehead{\chaptermark}
\chead{}
\rohead[]{\pagemark}
%\rohead{\pagemark}
%\lohead{\rightmark}
\lohead{\rightmark}
\rehead{\leftmark}
% \lehead{}
\lehead{\pagemark}
\lefoot{}
\cefoot[]{}
\cofoot[]{}
% \rofoot[\pagemark]{\pagemark}
\rofoot[]{}
\setheadsepline{1pt}

%%% Vertical offset of chapters (standard is 1.8)
\renewcommand*{\chapterheadstartvskip}{\vspace{2.2\baselineskip}}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "mainPhD"
%%% End: 

